Exploring the Design Space of Optical See-through AR Head-Mounted Displays to Support First Responders in the Field

First responders (FRs) navigate hazardous, unfamiliar environments in the field (e.g., mass-casualty incidents), making life-changing decisions in a split second. AR head-mounted displays (HMDs) have shown promise in supporting them due to its capability of recognizing and augmenting the challenging environments in a hands-free manner. However, the design space have not been thoroughly explored by involving various FRs who serve different roles (e.g., firefighters, law enforcement) but collaborate closely in the field. We interviewed 26 first responders in the field who experienced a state-of-the-art optical-see-through AR HMD, as well as its interaction techniques and four types of AR cues (i.e., overview cues, directional cues, highlighting cues, and labeling cues), soliciting their first-hand experiences, design ideas, and concerns. Our study revealed both generic and role-specific preferences and needs for AR hardware, interactions, and feedback, as well as identifying desired AR designs tailored to urgent, risky scenarios (e.g., affordance augmentation to facilitate fast and safe action). While acknowledging the value of AR HMDs, concerns were also raised around trust, privacy, and proper integration with other equipment. Finally, we derived comprehensive and actionable design guidelines to inform future AR systems for in-field FRs.

==> Figure_Layouts_Testing.tex <==
Firedept 3 Across

\begin{figure}
 \begin{subfigure}{0.32\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/Fire Intern Leveld.jpg}
  \caption{Fire Attack Training}
  \Description{A firefighter closes the window to the inside of the Fire Attack training building}
  \label{fig:FireAttack}
 \end{subfigure}
  \medskip %Image of Search & Rescue
 \begin{subfigure}{0.32\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/TIC Aspect Ratio.png}
  \caption{Search and Rescue Training}
  \Description{Several Firefighters are searching the smoke filled basement}
     \label{fig:SearchRescue}
 \end{subfigure} 
 \begin{subfigure}{0.32\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/NIST Fire Group Pixelated.png}
  \caption{Discussions after Fire Attack Training}
  \Description{A Group of firefighters meeting after Fire Attack training to discuss the feedback from the training}
  \label{fig:FireAttackDiscussions}
 \end{subfigure} 
 \hfill
 \begin{subfigure}{0.49\textwidth} %Image of Hostage SWAT
     \includegraphics[width=\textwidth]{Images/SWAT.PNG}
    \caption{Hostage Rescue Training}
    \Description{A Group of swat members disarm an assailant}
     \label{fig:HostageScenario}
 \end{subfigure}
 
 
 AR Augment Symbols 4 across
 
 \begin{figure}
 \begin{subfigure}{0.24\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/AR Features/Symbol Same Crop.png}
  \caption{Symbol}
  \Description{An example of a symbol hologram.}
  \label{fig:symbol}
 \end{subfigure} 
 \begin{subfigure}{0.24\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/AR Features/Arrow Same Crop.png}
  \caption{Arrow}
  \Description{An example of an arrow hologram for navigation.}
     \label{fig:arrow}
 \end{subfigure}
  \begin{subfigure}{0.24\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/AR Features/Door Highlight Same Crop.png}
  \caption{Highlight Object}
  \Description{An example of highlighting an object, specifically a door knob.}
  \label{fig:highilight}
 \end{subfigure} 
 \begin{subfigure}{0.24\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/AR Features/Map Same Crop.png}
    \caption{Map}
    \Description{An example of a map hologram.}
     \label{fig:map}
 \end{subfigure}
  \caption{AR augmentations from the demonstration video we showed first responders}
 \label{Label}
  \yuhang{these figures are a bit low contrast, especially the last one, can you adjust the images? Or retake the images from hololens instead of a screenshot from the video}
\end{figure}

 AR Augment Symbols 2 col 2 row
 
 \begin{figure}
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/AR Features/Symbol Same Crop.png}
  \caption{Symbol}
  \Description{An example of a symbol hologram.}
  \label{fig:symbol}
 \end{subfigure} 
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/AR Features/Arrow Same Crop.png}
  \caption{Arrow}
  \Description{An example of an arrow hologram for navigation.}
     \label{fig:arrow}
 \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/AR Features/Door Highlight Same Crop.png}
  \caption{Highlight Object}
  \Description{An example of highlighting an object, specifically a door knob.}
  \label{fig:highilight}
 \end{subfigure} 
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{Images/Edited Images/AR Features/Map Same Crop.png}
    \caption{Map}
    \Description{An example of a map hologram.}
     \label{fig:map}
 \end{subfigure}
  \caption{AR augmentations from the demonstration video we showed first responders}
 \label{Label}
  \yuhang{these figures are a bit low contrast, especially the last one, can you adjust the images? Or retake the images from hololens instead of a screenshot from the video}
\end{figure}

==> Sections/2.1-Related_Work-unused.tex <==
\section{Related Work}

%Add the number of FR they interviwed
%Comment the GAP between the papers, how they didn't show technology

\subsection{Understanding the Experiences of First Responders}
Various prior work has explored the challenges and needs of different types of first responders through interviews and observations. 
Most of such research focused on firefighters (FF). For example, Toups et al. performed an ethnographic investigation on six fire emergency responders and 38 students at a fire training school, revealing their challenges in different tasks, including information flow (radio communication, face-to-face communication), team coordination, emergent practices, and team cognition \cite{toups2007implicit}. Denef et al. conducted an empirical study with several FF over 6 months, where they looked at the purpose and properties of their FF tools. They found that FF used radio for communication, hose and searching algorithms for navigation, and air tanks for breathing \cite{denef2009letting}. 

Besides FF, researchers have also looked into other types of first responders. For example, Dawkins et al. used an exploratory mixed method to interview 193 first responders (COMMS, EMS, FF, and LE) and survey them to examine the future use of communication technology, such as real-time on-scene video, indoor mapping, and voice controls for hands-free input.~\cite{dawkins2021futuristic}. %Dawkins et al. interviewed 133 first responders (FF, EMS, and LE) and surveyed them to understand their experience and the needs to communicate efficiently and effectively. 
Nunavath et al. conducted semi-structured interviews with three LE, 15 FF, and two municipality officials to identify their information needs~\cite{nunavath2016identifying}. Kristensen et al.shadowing several FF, LE, and EMS in their daily jobs. %had 13 researchers participate in incident procedures, 4 researchers observed specialized trauma team training, and observed 2 videos of major incidents. 
They summarized the needs and challenges of EMS and produced designs for sharing triage information, victim location or identification, and remote access information collected by different kinds of
sensors~\cite{kristensen2006participatory}.  

Some research focuses on exploring the potential of specific technologies for first responders. For example, Amon et al. hosted a workshop with 38 attendees that were experts from the first responder community, thermal imaging manufacturers, and FF trainers to discuss strategies, technologies, procedures, and best practices to improve FF's safety and fire protection, as well as the effectiveness of thermal imaging and it's needs to be used in the fireground \cite{amon2005thermal}. Some researchers focused on the use of drones by first responders. Alon et al. interviewed three FF to understand the current usage and barriers of drones. They also conducted a focus group of nine FFs and a gesture elicitation study to investigate collocated human-drone interactions to support FF~\cite{alon2021drones}. Khan et al. conducted an exploratory study with 20 9-1-1 callers and FF to explore drone system designs that can aid FF during emergencies, along with their benefits and challenges~\cite{khan2019exploratory}. 

There has been limited research that studied the first responders' needs for AR devices. Specifically, Kapalo et al. conducted field studies where they interviewed and observed 35 FF and 3 emergency management personnel to understand how AR could be used to minimize required user input, increase data sharing, support visualization of spatial information, emphasize critical cues, filter and customize information presented to the incident commander, and allow for the prediction of dynamic incident changes\cite{kapalo2018sizing}.
Wilson et al. interviewed 50 FF about their needs for head-mounted displays and found several reasons why participants wouldn't want to use such devices since it blocks their lower vision, screen was not level,device seemed to delicate, and that is wouldn't work in cold weather\cite{wilson2005design}. However, this work only asked participants to imagine the experiences of using AR glasses and answer hypothetical questions.    
Chan et al.'s work was the only exception. They interviewed 21 first responders and gave them a Recon Jet eyewear to discuss their experiences and feedback \cite{chan2016erwear}. However, unlike AR glasses that can register virtual elements in the physical environment, the eyewear used in this study was consisted of a pair of sunglasses with a small display attached to the right eye. It functioned as an external phone screen in front of users' eyes instead of augmenting the physical world directly. The researchers also found that such  devices still required repeated attention switches between the display and the physical world. No research has explored first responders' hands-on experiences with state-of-the-art AR glasses. 
%however, the work only briefly gives an example of their preliminary findings..
%All these studies focused on either a specific task for multiple FR or General Needs for a single FR group, with most of the research for their needs/challenges being over a decade old at this point. 

\subsection{AR Technology to Support First Responders}
There has been extensive research in designing and creating technologies to support first responders in various tasks, including communication \cite{farnham2006observation, aedo2010end, prasanna2011evaluation, camp2000supporting, streefkerk2006designing, scholz2013concept, bergstrand2009using, neustaedter2019sharing, landgren2005supporting}, navigation \cite{klann2007lifenet,klann2011experience, steingart2005augmented, liu2010automatic, ramirez2010designing}, and information gathering and sharing \cite{jiang2004ubiquitous, betz2014emergencymessenger, kasnesis2022deep, streefkerk2008field, purohit2011sensorfly, beata2018real}. For example, Bergstrand et al. created a live response application on a Bambuser
service on mobile terminals that incorporated map services, live video support, and awareness features. They developed the application through hosting four iterative prototype workshops with FRS, the Emergency Paramedics Service (EPS) and the Traffic and Road Authorities (TRA)~\cite{bergstrand2009using}. Kasnesis et al. created a system for FRs' dogs. They created a back-mounted wearable device, which can recognize dog activity, barks, and provided the dog handler the dog's location through a mobile application~\cite{kasnesis2022deep}. Moreover, Liu et al. created an automatic and robust wearable breadcrumb system for indoor FF scenarios that dropped quarter-size
mote powered by a lithium battery~\cite{liu2010automatic}. 
However, most prior technologies for first responders are not based on AR platforms. 

%in both training and in-the-field tasks. We summarize the designs and technologies of prior work below.
% \subsubsection{Technology not using AR/VR}
% There are various other technology designs for FR's that do not include AR or VR. These designs are based on the duties, current technology uses, and needs/challenges of FRs. These designs mainly focus on improving the needs of communication, information gathering and sharing, and navigation. A brief overview of the technology, uses, and the solutions they solve are discussed.
% These designs are based on the duties\cite{toups2007implicit}, the current technology uses \cite{denef2009letting,katsadouros2022introducing,amon2005thermal}, and needs/challenges \cite{carafano2017preparing} of FRs. These designs mainly focus on improving the needs of communication\cite{dawkins2021futuristic, dawkins2018public}, information gathering and sharing\cite{nunavath2016identifying}, and navigation\cite{wilson2005design}. A brief overview of the uses for the different technology and the solutions they solve are summarized below.

% \textit{\textbf{Communication.}}
% Communication between first responders is an essential part of their job. With numerous software applications being developed to promote collaboration during disasters, coordinate FR's strategies, and detail emergency scene information to other FR's. Farnham et al. examined Groove, a peer-to-peer technology that promotes communication and data flow across locations in time-pressured situations across ephemeral groups by observing and interviewing individuals who deployed Groove and relief works who used it\cite{farnham2006observation}. Aedo et al. studied an emergency management information system called SIGAME through an empirical study by survey 32 emergency workers and focused on inter-agency cooperation\cite{aedo2010end}. Prasanna et al. sought to improve Fire and Rescue Services (FRSs) information systems, by evaluating a prototype with 86 individuals from the FRSs brigade that specialized in different aspects of FRSs and hosting a workshop\cite{prasanna2011evaluation}.Camp et al. performed an ethnographic-style investigation on previous FF literature to understand their communication and design a Fire Communication System\cite{camp2000supporting}.

% Several communication interfaces for FR technology have been studied in great detail as well. Streefkerk et al. studied how to design personal attentive user interfaces (PAUI) by proposing a user-centered design method based on previous literature and domain analyses\cite{streefkerk2006designing}. Scholz et al. derived a set of high level requirements to support communication by analyzing FF standard ways of communicating through conducting 15 workshops with FF. 

% With newer ways of communication becoming standard in FR's daily lives like video calling, there are requests of integrating it into their field of work. To facilitate these requests research has tried to incorporate live video feeds of emergencies to individuals off-scene or provide video details to FRs en-route to the emergency. Bergstrand et al. created the live response application that incorporates map services, live video support, and awareness features. They developed the application through hosting 4 iterative prototype workshops with FRS, the Emergency Paramedics Service (EPS) and the Traffic and Road Authorities (TRA)\cite{bergstrand2009using}. Neustaedter et al conducted an exploratory study 
% where they observed 3 9-1-1 Call Centers and interviewed 12 firefighters to understand how video information systems could be designed for FF and how to share 9-1-1 video call information to FF through dispatchers\cite{neustaedter2019sharing}. 

% Other design concepts to promote alternate forms of communication are making verbal communication persistent and improving communication to FR en-route to the scene. Landgren et al. conducted a field study with Sweden's FRS and used an ethnographical approach to study the enroute operations of FF\cite{landgren2005supporting}. Again landgren et al studied empirical data from two FR major incidents to investigate mobile phone interaction in time-critical emergency responses\cite{landgren2005supporting}.

% \textit{\textbf{Information Gather and Sharing}}
% FR are constantly sharing information during emergencies to resolve situations and support other FR's. Information sharing can be broken down into two categories, on-scene sharing and off-scene sharing. For on-scene information sharing, various research has sought to improve current information sharing technology or create new ones. Jiang et al. conducted interviews with 14 FF and observed 3 fire departments as they went about their daily functions to design Siren a peer-to-peer architecture that supports information gathering and distribution on fire scenes\cite{jiang2004ubiquitous}.

% Newer technology designs to boaster information sharing are often creations that enhance older technology or provide completely new information. Betz et al. design and evaluated a text based messaging tool to support radio communication for FF through design-case-studies\cite{betz2014emergencymessenger}. Kasnesis et al. created a system for search and rescue dog's that is a back-mounted wearable device, which can recognize dog activity,barks, and provide the dog handler the dog's location through a mobile application\cite{kasnesis2022deep}. The system was valuated in 2 search and rescues.  Streefkerk et al. created a location-based notification system (LBNS) for LE, using a mobile device. They had 30 LE field evaluate LBNS to test the efficiency, effectiveness and user experience of the device\cite{streefkerk2008field}. Purohit et al. created SensorFly a mobile aerial sensor network for indoor FF emergency scenarios, with the design rationales based off of prior research. They evaluated it in a computer simulation environment\cite{purohit2011sensorfly}. Beata el at. proposed a real-time fire monitoring system that send fire data to other FF which implemented an event-detection model and was tested on simulated data from a Fire Dynamics Simulator(FDS)\cite{beata2018real}. 

% \textit{\textbf{Navigation}}
% Navigating in the complex environments FR encounter can be quite the challenge. To protect and help orientate FR's, prior work has focused on maps or other forms of directional information.Klann et al. created the FireSim experience-prototyping approach to explore their navigational support system called LifeNet\cite{klann2007lifenet}, which they used in a field study with 15 FF\cite{klann2011experience}. Liu et al. created an automatic and robust breadcrumb system for indoor FF scenarios\cite{liu2010automatic}.Ramierez et al. created multiple devices that would act as landmarks for FF to following in emergencies, they performed several prototyping workshops with FF. Their final design settled on a device FF would carry and could place, they emitted lights, acoustic and radio signals for FF to find them\cite{ramirez2010designing}.


% Such as a Handheld device that provides blueprints \cite{jiang2004siren}, Micro-displays that contain building information and biometrics which attach to masks\cite{klann2011experience}, and a head-mounted display that provide maps and collect fire data\cite{steingart2005augmented}. To help navigation in other formats wearable mounted displays that provide arrow direction\cite{klann2007lifenet} , sensor breadcrumb trails that FR would follow\cite{liu2010automatic}, and throwable sensors that act as landmarks\cite{ramirez2010designing} have been researched. 

With the advancement of AR, researchers have recognized its potential in recognizing and augmenting the physical environment and providing necessary and real-time support for first responders in the field. In this section, we focus on summarizing the AR technology innovation for first responders in both training and in-the-field tasks. %the potential for this technology to alleviate the challenges and solve the needs of FR is a possibility, by enhancing training or supplementing in-the-field emergency tasks.

\subsubsection{AR/VR for First Responder Training.} An important factor for FR's is the need to be contextually aware of their surroundings in an emergency, and since VR obscures the surroundings, it is used for recreating training or designing solutions. For example, Klann et al. created a VR simulated board game that represented possible scenarios, which helped FFs express different choices in emergency scenarios by acting them out to formulate design solutions to the problems FF's had~\cite{klann2007playing}. %, which they explored through a workshop of 12 FF. 
Koutitas et al. simulated EMS Ambulance Busses (AMBUS) training in VR and AR to improve training performance and evaluate it against the current EMS AMBUS training~\cite{koutitas2021performance}. Sebillo et al. designed a system to integrate AR functions such as highlighting buildings and visual text summaries next to the buildings, thus training FR in acquiring familiarity with new technologies~\cite{sebillo2015use}.

% AR's ability to keep the visual surroundings and provide overlays on top allow for training simulations\cite{koutitas2021performance} or the ability to reenact old emergencies to prepare FR's for future ones \cite{sebillo2015use}.

\subsubsection{AR Technologies to Support In-the-field Tasks.} \yuhang{this section needs to be expanded since it's highly relevant to our work; need to have more thorough categorization. Maybe based on whether they involved FRs in the research.}
The usefulness of AR during emergencies has been an important topic of discussion for awhile \cite{arregui2021can}. There have been several prior works that focus on AR Technology for first responders \cite{nunes2017augmented,datcu2016handheld,streaminghelon, brunetti2015smart,wani2013augmented, steingart2005augmented}.
For example, Saindis et al. presented a system to intuitively control UAVs for FRs through single-hand gestures and visualize the UAVs’ camera feed with AR, which consisted of a live video player with stop and play functionality and  toggle button that can select the video source~\cite{sainidis2021single}. Kamat et al. designed a concept of using AR to display damaged building information onto real structures through virtual highlights and overlays, which can then be measured and interpreted by FRs~\cite{kamat2007evaluation}. Campos et al. created an AR mobile application to assist FR in emergencies by displaying points of interests and a mini-map. This application was preliminary evaluated by three navy members and five navy members for the final evaluation; each navy member had experience in emergency simulation exercises~\cite{campos2019mobile}. Overall, while there are plenty of research none of them have heavily involved FRs in the design process.
% Nunes et al. designed a system to support real time disaster management activities through AR wearable devices by gathering information and providing situational awareness through \cite{nunes2017augmented}. Datcu et al. explored the usability of an AR mobile system by conducting a user study of 3 forensic investigators where they used the system in a real forensic training environment. 
% Streaming et al. conducted semi-structured interviews with 2 FF to explore the challenges they faced. They designed an Helmet with integrated thermal images and AR visor, the design was evaluated by 10 FF. The AR view was simulated using a tablet. 
% Brunetti et al. designed the system Smart Augmented Field for Emergency (SAFE) to support FRs in-the-field using an AR wearable device that supports context awareness, communication, coordination, mission tracking, monitoring, and analysis\cite{brunetti2015smart}.
% Wani et al. discussed the design concepts of using AR to enhance the current workflow of FF by using mobile equipment integrated with adaptive context aware work environments\cite{wani2013augmented}.
% Steingart et al. interviewed 60 FF about their challenges and needs with current technology and later 3 FF chiefs for their opinions on the most important information in emergencies. They then designed and prototyped FireEye, a head-mounted display that attached to FF masks and provided a map, SmokeNet, a smoke sensor that would send smoke/temperature data to incident commanders, and an Electronic Incident Command System (eICS) that accepted the SmokeNet Information, had access to the maps, and could send text messages to the head-mounted displays\cite{steingart2005augmented}.


% With most prior work focusing on developing AR systems for FR without involving them in the design process\cite{kapalo2018sizing,wani2013augmented}, such as developing a Live Feed AR Interface component into a UAV system \cite{sainidis2021single} or using AR to overlay data onto live feeds in disasters to provide FR rapid assessments of hazards \cite{kamat2007evaluation}. Research that does include FR is only during the evaluation process\cite{siu2013sidebars}, or prototyping stages \cite{campos2019mobile}.A key point of these AR systems for FR's are the type of devices created, with many focusing on handheld devices\cite{kamat2007evaluation, nunes2017augmented} either by choice\cite{datcu2016handheld}, or to simulate AR capabilities for their prototype\cite{streaminghelon}. Only one prior work gave FR's a wearable AR device(i.e, The Recon Jet eyewear) to design rationales for AR, however only a brief example of their preliminary findings were discussed\cite{chan2016erwear}.

% The duties\cite{toups2007implicit}XXXXX and the technology use \cite{denef2009letting} XXXXXs of First Responders has been studied in various research. With their main focuses on how to improve navigation\cite{}, communication\cite{}, and information gathering\cite{} in both training and active emergencies. To facilitate these task designs and prototypes for different types of first responders have been created using a wide assortment of technology. Even the requirements for how the user interfaces\cite{beata2018real} \cite{streefkerk2006designing} should be, the goals/devices needed \cite{katsadouros2022introducing} XXXXX, and the challenges\cite{wani2013augmented} XXXXX \cite{landgren2007study}for creating such a system have been studied.
    
% Specific Techs and how they break down
%     With the advancement of AR/VR development this technology could be used to benefit first responders\cite{arregui2021can} \cite{kapalo2018sizing} XXXXX
%         Communication
%             Using drones to receive live feeds of the  emergency scene through a wearable device \cite{sainidis2021single} XXXX
%             Mobile AR application that marks points of interest for firefighters\cite{siu2013sidebars} XXXX
%             Mobile AR application that provides insights about the scene and shares information with other first responders\cite{campos2019mobile} Similar to 12 but this is for general first responders XXXX
%             VR board game that helps firefighters design how they should information share during scenarios \cite{klann2007playing} XXX
            
%         Information Gathering
%             Things like Simulating training through AR and VR to boost learning in the EMS field. \cite{koutitas2021performance} XXX
%             Overlaying data onto live feeds during disasters to provide rapid assessments of hazards\cite{kamat2007evaluation}XXXXX
%             AR interfaces to prepare first responders for real scenarios\cite{sebillo2015use} XXX
%             AR Mobile app to provide location, scene information, and suggest best course of actions to first responders while on scene\cite{nunes2017augmented} XXXXX
%             Handheld AR device that allows police to explore and mark interest objects during crimes scenes for others to view
%              \cite{datcu2016handheld} XXXX
%         Navigation
%             Helmet for firefighters that has thermal imaging, biometrics, zoom function, and orientation\cite{streaminghelon} XXXX
        
%     Information collection to gain a better understanding of the emergency.
%         Small areal devices to collect data of fire's before firefighters are sent into the buildings\cite{purohit2011sensorfly}
%         Real-time fire monitoring system placed in houses to remotely send data to others outside of the scene\cite{beata2018real}
%         Drones to follow firefighters into the scene to increase situation awareness\cite{alon2021drones} \cite{khan2019exploratory}
        
%     Enhancing communicating information among first responders
%         Design/Ideas Concepts
%             Design idea to make sharing information among firefighters visible and not have to use words \cite{landgren2006making}
%             Concept of making communication between firefighters easier \cite{scholz2013concept}
%             Allowing firefighters enroute to a scene to know of pressing information about it. Improves communication between incident commander and other firefighters\cite{landgren2005supporting} NO prototype just design ideas
            
%         Video Sharing
%             Sharing live video of emergencies to various agencies not on the scene \cite{bergstrand2009using}
%             Sharing live video details from 911 as they make their way to the scene \cite{neustaedter2019sharing}
            
%         System/Software Applications
%             Groove computer application that promotes collaboration during disasters \cite{farnham2006observation}
%             Computer Software that details important emergency scene information \cite{prasanna2011evaluation}
%             Information System to coordinate first responders and promote first responders to use similar strategies \cite{aedo2010end}
        
%         On Scene Information Sharing
%             Better information display for Firefighting Incident commands to track firefighters in the scene and other resources \cite{jiang2004ubiquitous}
%             Improving current radios at the time to allow easier communication between each hierarchy of firefighters on scene \cite{camp2000supporting}
%             Handheld device that allows firefighters to send messages to each other in the fire \cite{betz2014emergencymessenger}
%             Dog tracking for police officers to know the location of their dogs via a wearable device that has a camera. \cite{kasnesis2022deep}
            
%         Off scene Information Sharing    
%             Mobile application that notifies police officers of various details such as warrents and other pressing information \cite{streefkerk2008field}
%             Sharing victim information and triage information to those off scene for EMS \cite{kristensen2006participatory}

%     Providing Navigation methods to help with safety and orientation.
%         Maps
%             Handheld device that provides the blueprints of the current building which is on fire to the firefighters inside, automatic warnings from data collections, and warning messages from other teammates \cite{jiang2004siren}
%             Micro-display that provides information on how to get out of a building for firefighters and biometrics(heart rate, air) Similar to (15) \cite{klann2011experience} but this is a micro-display attached to mask because AR wasn't that advanced yet.
%             Head mounted display that provides a map of the building to firefighters \cite{wilson2005design} Similar to 20 but way older before AR
%             Second iterations of the head mounted display of a map, but this time provides a smoke detector for data collection  \cite{steingart2005augmented}
        
%         Object Following Navigation Trail/Landmarks/Arrows
%             Wearable mounted display with sensors onto firefighters masks to provide arrow directions \cite{klann2007lifenet}
%             A device attached to the back of firefighters that drops sensors(objects) to create a breadcrumb trail \cite{liu2010automatic}
%             Landmark idea using throwable sensors that firefighters could use to enhance navigation \cite{ramirez2010designing}
        
        


% Number of Papers: 45 (Need for Police/Medical)
%     Police 5
%     Medical 2
%     Firefighter 25
%     General 13

% Quick labeling of each paper in list(So Far)

% UnSorted and not in Related Work yet!!!!
% ERWear: Wearable System Design through the Lens of First \cite{chan} Responders  XXXX

% PUBLIC SAFETY COMMUNICATION USER NEEDS: VOICES OF FIRST RESPONDERS Design requirements of tech and comm XXXX

% Identifying First Responders Information Needs: Supporting Search and Rescue Operations for Fire Emergency Response,  needs for search and rescure XXXX

% THERMAL IMAGING RESEARCH NEEDS FOR FIRST RESPONDERS, needs for thermal imaging

% Preparing Responders to Respond: The Challenges
% to Emergency Preparedness in the 21st Century, challenges for first responders emergency XXXXXX
% What Futuristic Technology Means for First Responders: Voices from the Field XXXX

% Tech Architecture Papers
% 	1- Single-Handed Gesture UAV Control and Video Feed AR Visualization for First Responders (2021, General FR, Gesture for Drone flying, provides AR video feed of drone to user wearable device)
% 	2-Evaluation of Augmented Reality for Rapid Assessment of Earthquake-Induced Building Damage (2007, General FR, AR overlay structural damage data to live video feeds to earthquake, disasters)
% 	3-SensorFly: Controlled-mobile Sensing Platform for Indoor Emergency Response Applications (2011, firefighters, small areal like drones, go into buildings and collect data)
% 	4-Real-Time Fire Monitoring and Visualization for the Post-Ignition Fire State in a Building (2018, Firefighters, real-time fire monitoring system to collect data)
% 	5-LifeNet: an Ad-hoc Sensor Network and Wearable System to Provide Firefighters with Navigation Support(2007, Firefighter, wearable head mounted display/sensors provides navigation out of building through arrows)
% 	6-Introducing the Architecture of FASTER: A Digital Ecosystem for First Responder Teams(2022, General FR, Propose architecture of a Tech and the goals for it)
% 	7-Deep Learning Empowered Wearable-Based Behavior Recognition for Search and Rescue Dogs(2022,Police, wearable dog device for location, video feed)
% 	8-Automatic and Robust Breadcrumb System Deployment for Indoor Firefighter Applications(2010,Firefighters, Manual breadcrumb trail navigation)


% Design Papers with Tech/Prototype
% 	9-Using live video for information sharing in emergency response work (2009, General FR,live video sharing)
% 	10-Ubiquitous Computing for Firefighters: Field Studies and Prototypes of Large Displays for Incident Command (2004, Firefighters, paper map for Incident Commanders)
% 	11- Siren: Context-Aware Computing for Firefighting (2004, Firefighters, Handheld phone device gives map blueprint, automatic warnings, and warnings from fellow firefighters)
% 	12-SidebARs: Improving awareness of off-screen elements in mobile augmented reality (2013, Firefighters, Mobile AR app to show points of interest)
% 	13-Performance evaluation of AR/VR training technologies for EMS first responder (2018, EMS, VR/AR training application to simulate real training)
% 	14-Observation of Katrina/Rita Groove Deployment: Addressing Social and Communication Challenges of Ephemeral Groups (2006,General FR, Groove web application for communications during disasters review)
% 	15-Mobile Augmented Reality Techniques for Emergency Response (2019, General FR, AR mobile app to provide information about scenes to FR’s)
% 	16-The Use of Augmented Reality Interfaces for On-site Crisis Preparedness(2015,General FR, System design for AR interfaces to help simulated training scenarios for FR)
% 	17-Helon 360: A smart firefighters ’ helmet(2019, Firefighters, Wearable helmet integrates tick, orientation, zoom, air,heart rate)CLOSEST WORK
% 	18-Handheld Augmented Reality for Distributed Collaborative Crime Scene Investigation(2016, Police, AR Device to explore and mark crime scene and share it remotely)
% 	19-Field Evaluation of a Mobile Location-Based Notification System for Police Officers(2008, Police, Mobile App Map shows various important police information, warrents,locations)
% 	20-Experience Prototyping: A New Approach to Designing Firefighter Navigation Support(2012,Firefighter, Microdisplay and sensors, provides navigation out building using sensors, air,temp, heartrate)CLOSTEST WORK
% 	21-Evaluation of a Software Prototype for Supporting Fire Emergency Response(2011,Firefighters, Computer app details of scene)
% 	22-End-user oriented strategies to facilitate multi-organizational adoption of emergency management information systems(2009, General FR, app to coordinate FR)
% 	23-EmergencyMessenger: A Text based Communication Concept for Indoor Firefighting(2014,Firefighter,handheld device send/recieve messages)
%     24-Drones in Firefighting: A User-Centered Design Perspective(2021,Firefighters, use of drones in firefighting situations)
%     25-Designing for high expectations: Balancing ambiguity and thorough specification in the design of a wayfinding tool for firefighters(2010, Firefihters, throwable landmarks for navigation)
%     26-Design of monocular head-mounted displays for increased indoor firefighting safety and efficiency(2005, firefighters, manual head mounted display on mask for navigation)CLOSESET WORK  
%     27-Augmented Reality in Support of Disaster Response(2018,General FR, AR mobile app to provide locations, best course of actions, scene details to diaster responses)
%     28-Augmented cognition for fire emergency response: An iterative user study(2005,Firefighter, mounted wearable device on mask, provides map, smoke data)



% Design Papers/Explanations/Reviews with theoretical design ideas NO tech/prototype
% 	29-Supporting fire crew sensemaking enroute to incidents (2005, Firefighters, Improving information between fire crew and command)
% 	30-Supporting Communication and Collaboration Practices in Safety-Critical Situations (2000, Firefighters, everyone gets a radio for communication, better current radios, access to both officer and command info)
%     31-Sharing 9-1-1 Video Call Information between Dispatchers and Firefighters During Everyday Emergencies (2019, Firefighters, Viewing 911 video call information on the way to a scene)
%     32-Playing with Fire: User-Centered Design of Wearable Computing for Emergency Response (2007, Firefighters, VR game like board to create future designs for information sharing)
%     33-Participatory Design in Emergency Medical Service: Designing for Future Practice (2006, EMS, Designing a Biometric device to share information about victims at scene and locations remotely)
%     34-Making Action Visible in Time-critical Work(2006, Firefighters, observed firefighters, created designs ideas to better communication information)
%     35-Letting Tools Talk:Interactive Technology for Firefighting(2009, Firefighters, descriptions of current firefighter Tech)
%     36-Implicit Coordination in Firefighting Practice: Design Implications for Teaching Fire Emergency Responders(2007,Firefighters,overview of firefighting challenges they face)
%     37-How can AR be used to improve first responders operations: an overview(2021, General FR, Powerpoint on how AR could be beneficial to FR)
%     38-Generic functionality in user interfaces for emergency response(2011,General FR, Needs of FR for user Interfaces, Interviewed each group and found functional needs)
%     39-Designing personal attentive user interfaces in the mobile public safety domain(2006,Police, user interface designs for mobile app PDA police)
%     40-Designing Context-Aware HCI for Collaborative Emergency Management(2008,general FR, key challenges for designing a Emergency Management system)
%     41-Augmented Reality for Fire & Emergency Services(2013, Police & firefighters, AR app to provide x-ray vision, markers, Map blueprints, paths)CLOEST WORK 
%     42-An Exploratory Study of the Use of Drones for Assisting Firefighters During Emergency Situations(2019,firefighters, drone use in firefighting challenges)
%     43-A Study of Emergency Response Work:Patterns of Mobile Phone Interaction(2007,General FR, overview of mobile interactions among FR, designs, challenges)
%     44-A Concept for Support of Firefighter Frontline Communication(2013, Firefighters, Concept of making communication between firefighters easier, provides requirements for tech)
%     45-“SIZING UP” EMERGING TECHNOLOGY FOR FIREFIGHTING: AUGMENTED REALITY FOR INCIDENT ASSESSMENT(2018,Firefighters, ways AR could replace current Firefighting tech)
    
% %

